Cross-Edge Orchestration of Serverless Functions with Probabilistic Caching

Serverless edge computing adopts an event-based paradigm that provides back-end services on an as-used basis, resulting in efficient resource utilization. To improve the end-to-end latency and revenue, service providers need to optimize the number and placement of serverless containers while considering the system cost incurred by the provisioning. The particular reason for this circumstance is that frequently creating and destroying containers not only increases the system cost but also degrades the time responsiveness due to the cold-start process. Function caching is a common approach to mitigate the coldstart issue. However, function caching requires extra hardware resources and hence incurs extra system costs. Furthermore, the dynamic and bursty nature of serverless invocations remains an under-explored area. Hence, it is vitally important for service providers to conduct a context-aware request distribution and container caching policy for serverless edge computing. In this paper, we study the request distribution and container caching problem in serverless edge computing. We prove the proposed problem is NP-hard and hence difficult to find a global optimal solution. We jointly consider the distributed and resource constrained nature of edge computing and propose an optimized request distribution algorithm that adapts to the dynamics of serverless invocations with a theoretical performance guarantee. Also, we propose a context-aware probabilistic caching policy that incorporates a number of characteristics of serverless invocations. Via simulation and implementation results, we demonstrate the superiority of the proposed algorithm by outperforming existing caching policies in terms of the overall system cost and cold-start frequency by up to 62.1% and 69.1%, respectively.

==> chapters/bio.tex <==
% !TEX root = ../serviceFunctionChain.tex
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/chen.jpg}}]{Chen Chen}
is a Research Associate in the Distributed Information and Automation Laboratory at the University of Cambridge. His research interests are broadly in areas of serverless computing, cloud and edge computing, network resource orchestration, in-network computing, distributed systems and service chaining.
\end{IEEEbiography}
\vskip 0pt plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/manuel.jpg}}]{Manuel Herrera}
is a Senior Research Associate in Distributed Intelligent Systems at the University of Cambridge. His research focuses on the development of predictive analytics and complexity science for smart and resilient critical infrastructure such as transport, telecommunications, and water. He is a fellow of the Royal Statistical Society (RSS), a committee member of the RSS Special Interest Group in statistical engineering, and the recipient of the Frank Hansford-Miller fellowship 2021 in applied statistics, awarded by the Statistical Society of Australia (WA Branch).
\end{IEEEbiography}
\vskip 0pt plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/ge.jpg}}]{Ge Zheng} is a Research Associate in the Distributed Information and Automation Laboratory (DIAL) at the Institute for Manufacturing (IfM), Department of Engineering, University of Cambridge, UK. She received her PhD degree with full PhD scholarship in the Department of Computing and Informatics at the University of Bournemouth, UK, and MSc degree with Academic Excellence International Masters Scholarship in Electronic Engineering from the School of Computer Science and Electronic Engineering at the University of Essex. Her interest areas involve edge computing, supply chain risk prediction, pattern recognition and/or classification, intelligent transportation systems, and healthcare applications.
\end{IEEEbiography}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/liqiao.jpeg}}]{Liqiao Xia}
received the B.S. degree from South China Agricultural University in 2017, M.S. degree from Hong Kong University of Science and Technology in 2020. He is currently working towards a Ph.D. degree in the Department of Industrial and Systems Engineering at the Hong Kong Polytechnic University. His research interests include edge computing, knowledge graph and reliability analysis.
\end{IEEEbiography}
\vskip 0pt plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/zhengyang.png}}]{Zhengyang Ling}
is a Research Associate at the Distributed Information and Automation Laboratory in University of Cambridge. He earned his PhD from the University of Leeds and holds MSc and bachelor degrees from East China University of Science and Technology. With over three years of experience in the automotive industry, including roles at SAIC Motor and ChanganUK. His research interests are edge computing, wireless sensors and actuators, optical measurement and their applications.
\end{IEEEbiography}
\vskip 0pt plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/photo-wjt.jpg}}]{Jiangtao Wang}
received the PhD degree from Peking University, China, in 2015. He is currently an Associate Professor in the
Intelligent Healthcare Centre, Coventry University, UK. Before that, he was a lecturer with the School of Computing and Communications
at Lancaster University, UK. His research interest includes mobile and pervasive computing, crowdsensing/crowdsourcing, and digital health.
\end{IEEEbiography}

